Recommendations with Sparse Comparison Data: Provably Fast Convergence for Nonconvex Matrix Factorization

This paper provides a theoretical analysis of a new learning problem for recommender systems where users provide feedback by comparing pairs of items instead of rating them individually. We assume that comparisons stem from latent user and item features, which reduces the task of predicting preferences to learning these features from comparison data. Similar to the classical matrix factorization problem, the main challenge in this learning task is that the resulting loss function is nonconvex. Our analysis shows that the loss function exhibits (restricted) strong convexity near the true solution, which ensures gradient-based methods converge exponentially, given an appropriate warm start. Importantly, this result holds in a sparse data regime, where each user compares only a few pairs of items. Our main technical contribution is to extend certain concentration inequalities commonly used in matrix completion to our model. Our work demonstrates that learning personalized recommendations from comparison data is computationally and statistically efficient.

==> paper_sections/2a_generative_model_old.tex <==
Let there be $n_1$ users and $n_2$ items. 
Each user $u$ and each item $i$ has a $r$-dimensional feature vector. 
The inner product of these two feature vectors gives the utility (or score) $x^*_{u,i}$ that user $u$ has for item $i$. 
This modeling assumption implies that
the score matrix $X^* \in \Real{n_1 \times n_2}$ has rank $r$, and thus admits the following rank-$r$ SVD:
\begin{align}
    X^* = U^* \Sigma^* V^{*T},
\end{align}
where $U^* \in \Real{n_1 \times r}$ and $V^* \in \Real{n_2 \times r}$ are matrices that satisfy $U^{*T} U^* = V^{*T} V^* = I_r$, and $\Sigma^* \in \Real{r \times r}$ is a diagonal matrix with entries $\sigma_1^* \geq \ldots \geq \sigma_r^* > 0$. Let $\kappa \triangleq \sigma_1^*/\sigma_r^*$ denote the condition number of $\Sigma^*$.

Let $n = n_1 + n_2$. Define $Z^* \in \Real{n \times r}$ and $Y^* \in \Real{n \times n}$ as follows:
\begin{align}\label{eq:matrix_z}
    Z^* &= 
    \begin{bmatrix}
        U^* \\ V^*
    \end{bmatrix}
    \Sigma^{* 1/2}, \\ 
    Y^* &= Z^*Z^{*T} = 
    \begin{bmatrix}
        U^*\Sigma^*U^{*T} & X^*\\
        X^{*T} & V^*\Sigma^*V^{*T}
    \end{bmatrix}.
\end{align}
From here on, we shall refer to $Z^*$ as the ground-truth matrix. Note that the singular values of $Z^*$ are $\sqrt{2\sigma_1^*}, \ldots, \sqrt{2\sigma_r^*}$.

We are given a dataset $\Dataset$ where each data point represents a comparison made by a user between two items. The size of the dataset, \textit{i.e.,} the number of data points, is represented by $m$. We index the dataset by $k$. Each data point $\Dataset_k$ is of the form $((u; i, j), w)$ and is sampled randomly as follows. The user index $u$ is chosen uniformly at random from $[n_1]$. The pair of item indices $(i,j)$ is chosen uniformly at random from the set of $n_2(n_2-1)$ pairs of distinct items. The item pair $(i,j)$ is sampled independently from $u$. The triplets for different datapoints are sampled independently of each other.

The variable $w$ reflects the outcome of the comparison made by the user $u$ between items $i$ and $j$. In the \textit{noisy} setting, $w$ is an indicator for the outcome of the comparison; it is one if $i$ is chosen and zero if $j$ is chosen. Given a triplet $(u; i, j)$, $w$ is a Bernoulli random variable with parameter $g(x^*_{u,i} - x^*_{u,j})$, where $g: \Real{} \rightarrow (0,1)$ is a known \textit{link function} that translates real-valued preferences to a binary scale. In the \textit{noiseless} setting, $w$ is set to the expected value of the corresponding noisy case; \textit{i.e.}, $w = g(x^*_{u,i} - x^*_{u,j})$. 

In this work, we assume we are given noiseless data. We assume the link function is a smooth, strictly increasing function and is symmetric around zero in the following sense: $g(-x) = 1 - g(x)$. For example, $g(x)$ could be the logistic link function: $e^x/(1 + e^x)$; this is the link function found in the Bradley-Terry-Luce choice model. 

\subsubsection{Important Parameters}

 


\paragraph{Incoherence} For any matrix $Z$, let $\norm{Z}_{2, \infty}$ denote the maximum of the $\ell_2$ norm of its rows and let $\norm{Z}_{F}$ denote the Frobenius norm of $Z$. Define the \textit{incoherence parameter} of the ground-truth matrix as 
\begin{align}\label{eq:def_mu}
    \mu \triangleq n(\norm{Z^*}_{2, \infty}^2/\norm{Z^*}_{F}^2).
\end{align}
In principle, $\mu$ can take values from $1$ to $n$. However, the sample complexity worsens with $\mu$.

\paragraph{Link Function Bounds}  Let $I$ denote the interval {$[-{24 \mu (\norm{Z^*}_F^2}/{n}), {24 \mu (\norm{Z^*}_F^2}/{n})]$.} 
Let $\xi$ and $\Xi$ be lower and upper bounds for the following expression:
\begin{align}\label{eq:link_function_lower_bound}
    \xi &\triangleq  \min_{x \in I, y \in I} \frac{g'(x)g'(y)}{g(x)(1 - g(x))}, \\ 
    \Xi &\triangleq \max_{x \in I, y \in I} \frac{g'(x)g'(y)}{g(x)(1 - g(x))}. \label{eq:link_function_upper_bound}
\end{align}
By the assumptions on $g(\cdot)$ stated above, $\xi$ is strictly positive and $\Xi$ is finite.

For the logistic link function, $g'(x)=g(x)(1-g(x))$, which implies $\xi = g'(24 \mu (\norm{Z^*}_F^2/n))$ and $\Xi = 1/4$.
